Physics-guided Full Waveform Inversion using Encoder-Solver Convolutional Neural Networks

Full Waveform Inversion (FWI) is an inverse problem for estimating the wave velocity distribution in a given domain, based on observed data on the boundaries. The inversion is computationally demanding because we are required to solve multiple forward problems, either in time or frequency domains, to simulate data that are then iteratively fitted to the observed data. We consider FWI in the frequency domain, where the Helmholtz equation is used as a forward model, and its repeated solution is the main computational bottleneck of the inversion process. To ease this cost, we integrate a learning process of an encoder-solver preconditioner that is based on convolutional neural networks (CNNs). The encoder-solver is trained to effectively precondition the discretized Helmholtz operator given velocity medium parameters. Then, by re-training the CNN between the iterations of the optimization process, the encoder-solver is adapted to the iteratively evolving velocity medium as part of the inversion. Without retraining, the performance of the solver deteriorates as the medium changes. Using our light retraining procedures, we obtain the forward simulations effectively throughout the process. We demonstrate our approach to solving FWI problems using 2D geophysical models with high-frequency data.

==> pages/introduction.tex <==
\chapter{Introduction and Background}

\input{pages/paper_intro}
%Full Waveform Inversion (FWI) is a challenging inverse problem in which we estimate the wave propagation velocity of a given medium using observed wavefield data on the boundaries. Inverse problems of this type arise in seismic exploration of oil and gas reservoirs, earth sub-surface mapping, tunnel detection \cite{jiang2020detecting,yu2022frequency,wang2019efficient,monte2009radio}, ultrasound imaging \cite{bernard2017ultrasonictomography}, optical diffraction tomography \cite{soubies2017diffraction}, brain imaging \cite{guasch2020brain} and more. The velocity estimation is performed by fitting simulated data to the observed data, and is formulated as an optimization problem. This problem is solved by a descent algorithm which iteratively reduces the misfit between the observed and simulated data, and gradually updates the underlying velocity model accordingly. At each iteration, the data simulation is obtained by solving the wave equation (in time domain) or the Helmholtz equation (in the frequency domain) for multiple sources for a given velocity model. That is, in the frequency domain, which is the focus of our research, one needs to solve the Helmholtz equation for multiple right hand sides at each iteration.

%The efficient numerical solution of the Helmholtz equation with high and spatially dependent wavenumber is a difficult computational task. The linear system obtained from the discretization of the Helmholtz equation involves a very large, complex-valued, sparse and indefinite matrix. The equation is most difficult in three dimensions, where a direct solver is very memory-consuming and impractical in most scenarios. On the other hand, there are multiple available iterative methods to solve the equation, but they typically require many iterations at high wavenumber. Either way, the data simulations are highly cumbersome in FWI and are the main computational bottleneck of the inversion.

%Beyond the high computational costs of the forward simulations, FWI is a highly non-linear and ill-posed problem, especially in the absence of low-frequency data, which are hard to acquire because of physical limitation. Therefore, sophisticated regularization techniques \cite{eran2021extendedfwi}, loss functions \cite{johnson2016perceptualloss}, and careful minimization strategies \cite{eran2017traveltime} are often considered. Still, even after several years of research, the solution process of FWI is sensitive, tricky and cumbersome.

%In recent years, data-driven deep learning (DL) methods \cite{krizhevsky2017imagenet,lecun2015deep,szegedy2015going} have revolutionized many scientific fields, most notably computer vision and natural language processing. Inverse problems were also treated by DL, and FWI in particular, because of its difficulty and non-linearity. In the context of FWI, two main approaches are considered: (1) data-guided approaches (end-to-end) where deep networks are trained to consume data on the one hand and output a velocity model on the other \cite{wulin2019inversionnet,feng2023simplifying,Li2020}, and (2) physics-guided approaches where the data-fitting structure of the problem is kept and we make sure that the resulting model fits the observed data in simulations \cite{sanghvi2019embedding,colombo2023self}. Here, we focus on the physics-guided approach, since the first approach is highly dependent on the setup of the problem (locations of sources and receivers, types of media in the training set etc.) and is not flexible between different experiments. In the physics-guided approach we can be flexible with respect to the setup of the problem and we are faithful to the classical approach of fitting numerical simulations. That is, we will integrate the use of deep learning within the optimization process of solving FWI.

My first objective focuses on easing the computational requirements of simulating data throughout the inversion process. Namely, we will ease the computational bottleneck of solving the Helmholtz equation with the integration of a CNN-based solver. The CNN network
is integrated within a classical iterative solver of the Helmholtz equation, and is able to accelerate the convergence of the solver \cite{azulay2022multigrid}. During the inversion process the underlying solution, i.e. the estimated velocity model, gradually changes. Thus, we propose a tuning procedure to cope with these changes
and help keep the efficiency of our CNN-based solver throughout the whole inversion process.

In my second objective, we consider the issue of the ill-posedness of the FWI problem. That is, given some noisy observed data, there is more than one solution that approximately fits
the data. Therefore, in order to restrict the solution to be in the correct function space a regularization
term is often introduced to the optimization formulation.  In this work we aim to learn deep regularizers \cite{eliasof2023drip} that will
be combined with classical data-fitting approaches so that the tool will be more applicable to real-life
scenarios. Our aim is to construct a DL methodology for learning regularizers from the given data
without prior knowledge.

In my third objective we aim to solve the problem of tunnel detection using FWI formulation. In our research we will model the tunnel's pathway using a Parametric Level Set (PaLS) representation. The PaLS representation is a compact algebraically representation of level set functions. In our case, we will use ellipsoidal radial basis functions which was shown to have an extensive and rich expressiveness \cite{eliasof2020multimodal}. This representation will help reduce the computational cost of the inversion process and construct a robust process for detecting tunnels in subsurface domains. 


Finally, in my last objective,
I aim to improve the solution process of the Helmholtz equation by taking a classical (non-neural) approach, as DL methods have their weakenesses. I aim to apply the approach of multi-preconditioning \cite{greif2017gmres} for the acoustic Helmholtz equation. Namely, to combine two or more different preconditioners
such that they solve the problem in synergy, complementing each other to yield the best performance. For a start, we observe that Lippman Schwinger (LiS) preconditioner \cite{soubies2017efficient,pham2020three}, which operates by taking a constant wavenumber operator to precondition a spatially varying
wavenumber operator, can give better result if we change the LiS preconditioner between
iterations. In addition, we may combine this method, that has a global behavior but is
inefficient in highly heterogeneous media, with the (local) domain decomposition method, such that each sub-domain has less variability in the wavenumber.


We believe
that the combination of our novel approach based on integrating DL methodologies in the physics-guided approach, and
the multi-preconditioning approach, may lead to robust and efficient solvers for the FWI problem, and may open a path for the development of efficient solvers for other inverse problems. Furthermore, we show that with representation modification we are able to use FWI in various real-life applications.

\paragraph{Thesis Organization and Outline}
In the following sections, I describe the necessary background and methods I intend to apply, including the advances in
my work so far. First, in the next section I provide some general background that is joint for all my proposed work. Then, I describe each proposed method and provide a more detailed background relevant to each line of work. Specifically, in chapter \ref{section:CNN_FWI} I elaborate on the research that has been conducted as part of my M.Sc study. This is followed by proposed research directions for
the remainder of my time as a research student in sections \ref{section:deep_regularization} to \ref{section:multipreconditioning}. 


